DrafTS: Time-Aware Decomposition with Residual Correction for Time Series Modeling

Real-world time series contain evolving underlying dynamics with irregular variations that lack stable temporal patterns and are often referred to as noise. Existing methods address this mixture by filtering frequencies or suppressing noisy observations. They either miss temporal evolution or risk suppressing useful dynamics. We propose DrafTS, a model-agnostic framework that aims to reduce noise while preserving evolving dynamics through time-aware Decomposition with ResiduAl correction For Time Series. DrafTS uses features derived from instantaneous amplitude and frequency to guide decomposition into a primary component intended to capture underlying dynamics. A task-specific backbone models the primary component, while a lightweight correction module uses residual information to correct the backbone output. Across four time series modeling tasks, DrafTS improves six diverse backbones, demonstrating its effectiveness. Code is at https://github.com/Autumn61q/DrafTS

==> tables/full_result_short_forecasting.tex <==
\newcommand{\best}[1]{\textcolor{red}{\textbf{#1}}}
\begin{table*}[t]
\centering
\vspace{-8pt}
\caption{
Short-term forecasting results on the M4 dataset.
Lower values indicate better performance.
The better result within each Raw/$+$Ours pair is highlighted in
\textcolor{red}{\textbf{red}}.
}
\label{tab:m4_full_results}
\small
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.08}

\resizebox{\textwidth}{!}{
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Dataset}
& \multirow{2}{*}{Metric}
& \multicolumn{2}{c|}{Crossformer}
& \multicolumn{2}{c|}{PatchTST}
& \multicolumn{2}{c|}{iTransformer}
& \multicolumn{2}{c|}{TimeMixer}
& \multicolumn{2}{c|}{TimeFilter}
& \multicolumn{2}{c}{LDrive} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
& & Raw & $+$Ours
  & Raw & $+$Ours
  & Raw & $+$Ours
  & Raw & $+$Ours
  & Raw & $+$Ours
  & Raw & $+$Ours \\
\midrule

\multirow{3}{*}{Yearly}
& sMAPE
& 15.369 & \best{15.059}
& 13.926 & \best{13.859}
& 14.076 & \best{14.023}
& 15.343 & \best{15.169}
& \best{13.996} & 14.032
& 14.076 & \best{13.896} \\

& MASE
& 3.571 & \best{3.442}
& 3.177 & \best{3.125}
& 3.169 & \best{3.159}
& 3.450 & \best{3.368}
& 3.115 & \best{3.111}
& 3.177 & \best{3.102} \\

& OWA
& 0.919 & \best{0.894}
& 0.826 & \best{0.817}
& 0.829 & \best{0.827}
& 0.904 & \best{0.888}
& \best{0.820} & 0.821
& 0.830 & \best{0.815} \\

\midrule

\multirow{3}{*}{Quarterly}
& sMAPE
& \best{11.467} & 11.588
& \best{10.640} & 10.664
& 10.834 & \best{10.741}
& 12.686 & \best{12.048}
& 11.289 & \best{10.971}
& 11.151 & \best{10.899} \\

& MASE
& \best{1.302} & 1.369
& \best{1.257} & \best{1.257}
& 1.260 & \best{1.251}
& 1.552 & \best{1.460}
& 1.326 & \best{1.264}
& 1.371 & \best{1.306} \\

& OWA
& \best{0.995} & 1.025
& \best{0.942} & \best{0.942}
& 0.951 & \best{0.944}
& 1.142 & \best{1.079}
& 0.996 & \best{0.959}
& 1.006 & \best{0.971} \\

\midrule

\multirow{3}{*}{Monthly}
& sMAPE
& 14.388 & \best{14.011}
& 13.329 & \best{13.241}
& 13.493 & \best{13.478}
& 14.200 & \best{14.127}
& 14.397 & \best{14.014}
& 14.043 & \best{13.883} \\

& MASE
& 1.102 & \best{1.086}
& 1.000 & \best{0.993}
& 1.019 & \best{1.017}
& 1.109 & \best{1.106}
& 1.087 & \best{1.046}
& 1.038 & \best{1.026} \\

& OWA
& 1.017 & \best{0.996}
& 0.932 & \best{0.926}
& 0.947 & \best{0.945}
& 1.013 & \best{1.010}
& 1.010 & \best{0.978}
& 0.975 & \best{0.964} \\

\midrule

\multirow{3}{*}{Others}
& sMAPE
& 5.719 & \best{5.223}
& 4.942 & \best{4.925}
& \best{4.807} & \best{4.807}
& 5.145 & \best{5.072}
& \best{5.136} & 5.224
& \best{4.770} & 4.829 \\

& MASE
& 4.013 & \best{3.617}
& \best{3.268} & 3.296
& \best{3.198} & 3.219
& \best{3.506} & 3.535
& \best{3.445} & 3.558
& \best{3.210} & 3.317 \\

& OWA
& 1.235 & \best{1.120}
& \best{1.035} & 1.038
& \best{1.010} & 1.013
& 1.094 & \best{1.091}
& \best{1.084} & 1.111
& \best{1.008} & 1.031 \\

\midrule

\multirow{3}{*}{\shortstack{\textbf{Weighted}\\\textbf{Average}}}
& \textbf{sMAPE}
& 13.479 & \best{13.231}
& 12.402 & \best{12.349}
& 12.554 & \best{12.513}
& 13.647 & \best{13.415}
& 13.096 & \best{12.848}
& 12.893 & \best{12.717} \\

& \textbf{MASE}
& 1.864 & \best{1.822}
& 1.676 & \best{1.662}
& 1.680 & \best{1.676}
& 1.873 & \best{1.833}
& 1.729 & \best{1.699}
& 1.718 & \best{1.685} \\

& \textbf{OWA}
& 0.984 & \best{0.964}
& 0.895 & \best{0.890}
& 0.902 & \best{0.900}
& 0.993 & \best{0.974}
& 0.935 & \best{0.918}
& 0.925 & \best{0.909} \\

\bottomrule
\end{tabular}
}
\vspace{-5pt}
\end{table*}

==> tables/main_result_cls.tex <==
\begin{table}[t]
\centering
\small
\caption{Classification results on 10 UEA datasets. Accuracy is reported as the mean and standard deviation over three seeds. Win, tie, and loss are counted over datasets.}
\label{tab:main_result_classification}

\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}

\newcommand{\gc}{\cellcolor{gray!10}}
\newcommand{\win}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\secbest}[1]{\textcolor{blue}{\underline{#1}}}
\newcommand{\imp}[1]{\,($+$#1)}
\newcommand{\negimp}[1]{\,(#1)}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|l|cc|ccc}
\toprule
& \multirow{2}{*}{\textbf{Backbone}}
& \multicolumn{2}{c|}{\textbf{Average Accuracy (\%)}}
& \multirow{2}{*}{\textbf{Win}}
& \multirow{2}{*}{\textbf{Tie}}
& \multirow{2}{*}{\textbf{Loss}} \\
\cmidrule(lr){3-4}
& & \textbf{Raw} & \textbf{+Ours} & & & \\
\midrule

\multirow{6}{*}{\shortstack{UEA\\(10 datasets)}}
& Crossformer
& \secbest{67.65$\pm$0.56}
& \gc\win{68.72$\pm$0.71}\imp{1.58\%}
& 9 & 1 & 0 \\

& PatchTST
& \secbest{68.31$\pm$0.19}
& \gc\win{68.87$\pm$0.66}\imp{0.82\%}
& 6 & 1 & 3 \\

& iTransformer
& \secbest{72.84$\pm$0.89}
& \gc\win{74.93$\pm$0.49}\imp{2.87\%}
& 10 & 0 & 0 \\

& TimeMixer
& \secbest{45.41$\pm$0.71}
& \gc\win{53.12$\pm$2.14}\imp{16.98\%}
& 9 & 1 & 0 \\

& TimeFilter
& \secbest{69.16$\pm$0.21}
& \gc\win{70.07$\pm$1.05}\imp{1.32\%}
& 9 & 0 & 1 \\

& L-Drive
& \secbest{46.03$\pm$0.52}
& \gc\win{48.74$\pm$0.54}\imp{5.89\%}
& 9 & 0 & 1 \\

\midrule
& \textbf{Average}
& \secbest{61.57$\pm$0.16}
& \gc\win{64.08$\pm$0.09}\imp{4.07\%}
& 52 & 3 & 5 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/main_result_short_forecasting.tex <==
\begin{table*}[thbp]
    \centering
    \vspace{-10pt}
    \caption{\textbf{Short-term forecasting results averaged over the six
    M4 subsets.} The cells highlighted in \colorbox{gray!10}{gray} report
    the results of \method{} (+Ours). The last row reports the average
    relative improvement in \textbf{sMAPE / MASE / OWA}.}
    \label{tab:main_result_short_forecasting}

    \setlength{\tabcolsep}{2.5pt}
    \renewcommand{\arraystretch}{1.05}

    \newcommand{\gc}{\cellcolor{gray!10}}
    \newcommand{\win}[1]{\textcolor{red}{\textbf{#1}}}
    \newcommand{\secbest}[1]{\textcolor{blue}{\underline{#1}}}
    \newcommand{\imp}[1]{\,(+$#1$)}
    \newcommand{\negimp}[1]{\,($#1$)}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}c cc cc cc cc cc cc@{}}
        \toprule

        \multirow{2}{*}{\textbf{Metric}}
        & \multicolumn{2}{c}{Crossformer \citeyearpar{crossformer}}
        & \multicolumn{2}{c}{PatchTST \citeyearpar{patchtst}}
        & \multicolumn{2}{c}{iTransformer \citeyearpar{itransformer}}
        & \multicolumn{2}{c}{TimeMixer \citeyearpar{timemixer}}
        & \multicolumn{2}{c}{TimeFilter \citeyearpar{timefilter}}
        & \multicolumn{2}{c}{L-Drive \citeyearpar{ldrive}} \\

        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
        \cmidrule(lr){10-11}
        \cmidrule(lr){12-13}

        & Raw & $+$Ours
        & Raw & $+$Ours
        & Raw & $+$Ours
        & Raw & $+$Ours
        & Raw & $+$Ours
        & Raw & $+$Ours \\

        \midrule

        sMAPE
        & \secbest{13.479}
        & \gc \win{13.231}\imp{1.84\%}
        & \secbest{12.402}
        & \gc \win{12.349}\imp{0.43\%}
        & \secbest{12.554}
        & \gc \win{12.513}\imp{0.33\%}
        & \secbest{13.647}
        & \gc \win{13.415}\imp{1.70\%}
        & \secbest{13.096}
        & \gc \win{12.848}\imp{1.89\%}
        & \secbest{12.893}
        & \gc \win{12.717}\imp{1.36\%} \\

        MASE
        & \secbest{1.864}
        & \gc \win{1.822}\imp{2.21\%}
        & \secbest{1.676}
        & \gc \win{1.662}\imp{0.84\%}
        & \secbest{1.680}
        & \gc \win{1.676}\imp{0.24\%}
        & \secbest{1.873}
        & \gc \win{1.833}\imp{2.17\%}
        & \secbest{1.729}
        & \gc \win{1.699}\imp{1.71\%}
        & \secbest{1.718}
        & \gc \win{1.685}\imp{1.92\%} \\

        OWA
        & \secbest{0.984}
        & \gc \win{0.964}\imp{2.02\%}
        & \secbest{0.895}
        & \gc \win{0.890}\imp{0.63\%}
        & \secbest{0.902}
        & \gc \win{0.900}\imp{0.28\%}
        & \secbest{0.993}
        & \gc \win{0.974}\imp{1.93\%}
        & \secbest{0.935}
        & \gc \win{0.918}\imp{1.80\%}
        & \secbest{0.925}
        & \gc \win{0.909}\imp{1.63\%} \\

        % \midrule

        % \textbf{Avg. Imp.}
        % & --
        % & \gc \textbf{\imp{2.02\%}}
        % & --
        % & \gc \textbf{\imp{0.63\%}}
        % & --
        % & \gc \textbf{\imp{0.28\%}}
        % & --
        % & \gc \textbf{\imp{1.93\%}}
        % & --
        % & \gc \textbf{\imp{1.80\%}}
        % & --
        % & \gc \textbf{\imp{1.64\%}} \\

        \bottomrule
    \end{tabular}
    }
    \vspace{-5pt}
\end{table*}
